X-Ray-to-Radio Offset Inference from Low-Count X-Ray Jets

Observations of positional offsets between the location of X-ray and radio features in many resolved, extragalactic jets indicates that the emitting regions are not co-spatial, an important piece of evidence in the debate over the origin of the X-ray emission on kpc scales. The existing literature is nearly exclusively focused on jets with sufficiently deep Chandra observations to yield accurate positions for X-ray features, but most of the known X-ray jets are detected with tens of counts or fewer, making detailed morphological comparisons difficult. Here we report the detection of X-ray-to-radio positional offsets in 15 extragalactic jets from an analysis of 22 sources with low-count Chandra observations, where we utilized the Low-count Image Reconstruction Algorithm (LIRA). This algorithm has allowed us to account for effects such as Poisson background fluctuations and nearby point sources which have previously made the detection of offsets difficult in shallow observations. Using this method, we find that in 55 % of knots with detectable offsets, the X-rays peak upstream of the radio, questioning the applicability of one-zone models, including the IC/CMB model for explaining the X-ray emission. We also report the non-detection of two previously claimed X-ray jets. Many, but not all, of our sources, follow a loose trend of increasing offset between the X-ray and radio emission, as well as a decreasing X-ray to radio flux ratio along the jet.

==> _unused_offset_mechanism.tex <==
The nature of a knot has been a matter of debate for a long time. They were described as re-confinement shocks \citep[e.g.,][]{komissarov1998large,laing2002dynamical} or internal shocks at jet-bending on kpc-scales \citep[e.g.,][]{2005MNRAS.360..926W} or moving features \citep[e.g.,][]{stawarz2004multiwavelength,kataoka2008chandra} within the jet flow. Moreover, the question of what produces an offset in a knot is still uncertain. Below we briefly describe and evaluate the applicability of two models that attempted to explain the observed offsets.

\subsection{Synchrotron time lags model}
\begin{figure*}
    \gridline{
        \fig{images/misc/Contour_0.1G.pdf}{0.5\textwidth}{(a)}
        \fig{images/misc/Contour_0.1G_2x.pdf}{0.5\textwidth}{(b)}
    }
    \gridline{
        \fig{images/misc/Contour_1mG.pdf}{0.5\textwidth}{(c)}
        \fig{images/misc/Contour_1mG_2x.pdf}{0.5\textwidth}{(d)}
    }
\caption{Plots of viewing angle vs. bulk Lorentz factor of the jet for the synchrotron time lag model. The top panel shows the results for a magnetic field of 0.1 mG with the LIRA measured offsets to the left and two times the offsets to the right. The bottom panel shows the same results as the top panel but with a magnetic field of 1 mG. In all the cases, the model requires the jet to be aligned to less than 10 degrees for $\Gamma=2$, which is highly unlikely (see text for details).  (\label{fig:time_lag_model}}
\end{figure*} 
In this model, originally proposed by \citet{bai2003radio}, the authors have assumed that internal shocks produce the knots on kpc scales. Shock accelerated electrons while propagating downstream along the jet would cool via synchrotron mechanism and progressively emit at lower frequencies. Hence, higher frequency radiation appears closer to the core when compared to their lower-frequency counterparts. The projected X-ray-to-optical offset is given by \citep[Equation 13 in][]{bai2003radio}
\begin{equation}
\label{eq:dxo}
    D_{x/o}\approx144 B^{-3/2}\beta\Gamma[\delta/(1+z)]^{1/2} \sin{\theta}~\text{pc}
\end{equation}
and the projected X-ray-to-radio offset \citep[Equation 14 in][]{bai2003radio} is given by
\begin{equation}
\label{eq:dxr}
    D_{x/r}\approx193 B^{-3/2}\beta\Gamma[\delta/(1+z)]^{1/2} \sin{\theta}~\text{kpc}
\end{equation}
where B is the magnetic field (in units of $10^{-4}$~G), $\Gamma$ is the bulk Lorentz factor of the jet, $\delta$ is the Doppler beaming factor and z is the redshift. We did not assume a single speed for the jet to evaluate this model over a range of bulk Lorentz factors and viewing angles. Hence, our equations slightly differ from their original form. 

Although an offset computed using LIRA may not always indicate the true offset, it provides a lower limit. We first checked whether these lower limits required reasonable viewing angle and bulk Lorentz factor using typical magnetic field values of 0.1~mG and 1~mG \citep[e.g.,][]{harris2002x,kataoka2005x,worrall2009x}. Note that the maximum deprojected offsets range from \siml4 kpc at lower redshifts \citep{kataoka2008chandra} to \siml7 kpc at higher redshifts \citep{2007ApJ...657..145S}. As the maximum observed offset in our sample is about \siml4 kpc (3C 275.1), we also scaled the offsets by two and re-derived the parameters. We show the results in Figure \ref{fig:time_lag_model}. In many cases, even for a moderate bulk Lorentz factor of 1.25 \citep[e.g.,][]{wardle1997fast}, the model requires that the jets be aligned $\lesssim10$~deg to our line of sight. Because the observed offset is inversely proportional to $B^{3/2}$, if we adopt a magnetic field smaller than 0.1 mG, the viewing angle is constrained to an even smaller value. However, the presence of offsets in FR-II and LDQ type sources indicates that it is highly unlikely for all the jets to be aligned at $\lesssim10$~deg.


Furthermore, the X-ray-to-optical offset (Eq.~\ref{eq:dxo}) is approximately three orders of magnitude smaller than the X-ray-to-radio offset (Eq.~\ref{eq:dxr}). That means the X-ray peak would almost coincide with its optical counterpart. However, HST images of 3C 17 presented in \citet{Massaro_2009} show that the optical emission coincides with the radio peak in knot S11.3. At the same time, our analysis also reveals an Xf offset, thereby ruling out the synchrotron time-lag model for this source.

\citet{bai2003radio} also noted that the transverse expansion of the jet could reduce the observed offsets as the electrons would also have to propagate in the transverse direction additionally. However, this effect may not be significant on scales of a few kpc \citep[e.g.,][]{kataoka2008chandra} and hence cannot explain the small observed offsets.

\subsection{Knots as moving blobs of plasma}
Alternative to the re-confinement shocks, knots were also modeled as fast moving parts of plasma surrounded by a slow otherwise identical outflow \citep[e.g.,][]{bridle1986collimation,stawarz2004multiwavelength}. These knots would be produced by an intermittent activity of the central engine. In this case, a forward-reverse shock could form at the downstream tip of the knot. The forward shock produces radio emission while the reverse shock produces X-rays, thereby creating an Xf-offset \citep{kataoka2008chandra}. Despite the consistency of the observed offsets in 3C 353 with the estimated intermittent activity time scales of $\approx10^4-10^5$~yrs \citep[e.g.,][]{reynolds1997intermittent,clarke1992origin}, \citet{kataoka2008chandra} note a few problems with this model. First, it is not clear why the two shocks should produce two seemingly different electron populations. Second, there is no reason why the structure of offsets in knots and hotspots should be similar. These problems led them to propose that the knots are instead heavier (relativistically) and slow moving blobs of plasma surrounded by a fast outflow. In this scenario, a single reverse shock forms at the upstream end of the blob that propagates in the faster outflow and produces X-rays; the radio emission would coincide with the blob. Here the forward shock would be nullified because of the assumed high-density ratio of the blob.

\begin{figure*}
    \gridline{
        \fig{images/misc/Contour_time_scales_1kpc.pdf}{0.5\textwidth}{(a)}
        \fig{images/misc/Contour_time_scales_4kpc.pdf}{0.5\textwidth}{(b)}
    }
\caption{Plot of viewing angle vs. bulk Lorentz factor of the contact discontinuity for a projected offset of 1 kpc (left) and 4 kpc (right). For the heavy moving knot model, it is assumed that the contact discontinuity is at rest in the knot's reference frame.  \label{fig:moving_knot_lag_model}}
\end{figure*} 


In the fast moving knot model, the distance between forward and reverse shocks is given by \citep[for example, Eq. E4 in][]{stawarz2004multiwavelength}:
\begin{equation}
    \Delta l = 2c\beta_{sh}^{\prime} \frac{\delta_{ct}}{\Gamma_{ct}}\Delta t
\end{equation}
where $\delta_{ct}$ and $\Gamma_{ct}$ are the Doppler factor and bulk Lorentz factor of the contact discontinuity in the observer's frame respectively and $\beta^\prime_{sh}$ is the speed of the shock in the contact frame. Adopting $\beta_{sh}^{\prime}=0.19$ from \citet{kataoka2008chandra}, the time scale is given by 
\begin{equation}
\label{eq:delta_t}
    \Delta t\sim8\times10^3 (\Delta l) \frac{\Gamma_{ct}}{\delta_{ct}}
\end{equation} 
where $\Delta l$ is the deprojected length in kpc. All our offsets are on the order of a few kpc, and the resulting time scales are approximately consistent with the estimated values of the intermittent jet activity. But because the measured offsets are lower limits and are projected on to the sky, the estimates of the time scales using LIRA derived offsets are also lower limits.

For various time scales, we show possible values of $\Gamma_{ct}$~and~$\theta$~for projected offsets of 1 kpc and 4 kpc in Fig.~\ref{fig:moving_knot_lag_model}. If the actual knots in jets are composed of moving knots, we may not notice offsets in many jets simply because of the associated time scales and projection effects. For example, for a jet located at a redshift of 0.5 (1\as= 6.7 kpc) and aligned at an angle of 20 deg to our line of sight, an offset of 1 kpc (\siml0.15\as) can only be observed on a time scale of $\approx10^5$~yrs (see Fig.~\ref{fig:moving_knot_lag_model}a) and \textit{ Chandra} may not resolve such an offset. If we were to observe an offset of 4 kpc (\siml0.6\as), the associated time scale becomes $\sim10^6$~yrs, which is within a factor of a few (see Fig.~\ref{fig:moving_knot_lag_model}b) of the typical age of a jet itself \citep[e.g.,][]{harwood2012determines}. Hence, it is possible that we may not have detected all the offsets  because a large fraction of deep \textit{Chandra} observations are quasars, which have closely aligned jets.

In the simplest scenario, we can also apply Eq.~\ref{eq:delta_t} to a heavier ans slow blob that moves in a fast outflow. However, the shocks will not be symmetric in the frame of the contact discontinuity. Hence the estimate will be larger by a factor of two. We also do not know whether a travelling shock could sustain for such long times and it could reduce the observed offset. Moreover, the heavier blob will act as a reflecting wall leading to a different shock speed. The original model suggested that a moving blob would represent a radio knot. That means a radio knot would appear as a volumetric feature contrary to the observations that radio knots represent a surface-emitting feature \citep{swain1997multifrequency,swain1998internal}. Within the context of the heavy blob model, it is possible that that the fast outflow flows \textit{around} the heavier blob creating a shear layer. This shear layer can accelerate the electrons to produce radio emission. Further analytical and numerical work is necessary to confirm this and other speculations.


\subsection{Jet-bending and internal shocks}


==> fig3set.tex <==
\figsetstart
\figsetnum{3}
\figsettitle{Results for the analysis of 22 sources}

\figsetgrpstart
\figsetgrpnum{3.1}
\figsetgrptitle{3C 6.1}
\figsetplot{3C6.1_lira_paper_count.eps}
\figsetplot{3C6.1_lira_paper_add.eps}
\figsetplot{3C6.1_lira_paper_offset.eps}
\figsetplot{3C6.1_NHS_lira_post.pdf}
\figsetplot{3C6.1_SHS_lira_post.pdf}
\figsetgrpnote{Results for the analysis of 3C 6.1, an FR-II NLRG--with the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component. (c) Same as (a) and (b) but zoomed in to NHS (top) and SHS (bottom) respectively. The Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-rays peak closer to the core than the radio in NHS. The jet appears to make a 90 deg turn to the west before reaching SHS where the X-rays peak upstream of the radio. (d)-(e) The distributions of $\xi$ in each ROI  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{1.5, 8, 15, 40}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.2}
\figsetgrptitle{3C 17}
\figsetplot{3C17_lira_paper_count.eps}
\figsetplot{3C17_lira_paper_add.eps}
\figsetplot{3C17_S3.7_lira_post.pdf}
\figsetplot{3C17_S11.3_lira_post.pdf}
\figsetplot{3C17_S10.8_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for 3C 17, an FR-II BLRG. \Radiocontours{5, 10, 20, 40, 80}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.3}
\figsetgrptitle{3C 133}
\figsetplot{3C133_lira_paper_count.eps}
\figsetplot{3C133_lira_paper_add.eps}
\figsetplot{3C133_B_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 133, a HERG. \Radiocontours{ 2, 4, 8, 10, 20, 40, 80}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.4}
\figsetgrptitle{0529+075}
\figsetplot{0529+075_lira_paper_count.eps}
\figsetplot{0529+075_lira_paper_add.eps}
\figsetplot{0529+075_B_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 0529+075, a highly-superluminal CDQ.  \Radiocontours{1, 2, 3, 4, 8, 20, 100, 1000}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.5}
\figsetgrptitle{3C 179}
\figsetplot{3C179_lira_paper_count.eps}
\figsetplot{3C179_lira_paper_add.eps}
\figsetplot{3C179_knot_lira_post.pdf}
\figsetplot{3C179_HS_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 179, an LDQ. \Radiocontours{ 0.3, 2, 4, 8}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.6}
\figsetgrptitle{4C+25.21}
\figsetplot{4C+25.21_lira_count.eps}
\figsetplot{4C+25.21_lira_add.eps}
\figsetplot{4C+25.21_B_post.pdf}
\figsetplot{4C+25.21_C_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for 4C+25.21, a high redshift quasar. \Radiocontours{0.5, 2, 4, 8, 20}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.7}
\figsetgrptitle{TXS 0833+585}
\figsetplot{TXS0833+585_lira_paper_count.eps}
\figsetplot{TXS0833+585_lira_paper_add.eps}
\figsetplot{TXS0833+585_A_lira_post.pdf}
\figsetplot{TXS0833+585_B_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for TXS 0833+585, a high-redshift quasar. \Radiocontours{0.34, 0.5, 2, 20, 200}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.8}
\figsetgrptitle{3C 213.1}
\figsetplot{3C213.1_lira_paper_count.eps}
\figsetplot{3C213.1_lira_paper_add.eps}
\figsetplot{3C213.1_NHS_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for 3C 213.1, an LERG. \Radiocontours{0.5, 2, 8, 40}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.9}
\figsetgrptitle{3C 220.2}
\figsetplot{3C220.2_lira_paper_count.eps}
\figsetplot{3C220.2_lira_paper_add.eps}
\figsetplot{3220.2_shs_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for 3C 220.2, a quasar. \Radiocontours{0.5, 2, 5, 20, 80}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.10}
\figsetgrptitle{4C+55.17}
\figsetplot{4C+55.17_lira_paper_count.eps}
\figsetplot{4C+55.17_lira_paper_add.eps}
\figsetplot{4C+55.17_A_lira_post.pdf}
\figsetplot{4C+55.17_HS_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for 4C+55.17, a quasar/FSRQ. \Radiocontours{2, 4, 8, 40, 100, 1000}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.11}
\figsetgrptitle{PKS 1046-409}
\figsetplot{PKS1046-409_lira_paper_count.eps}
\figsetplot{PKS1046-409_lira_paper_add.eps}
\figsetplot{PKS1046-409_C_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the ATCA 19 GHz radio contours overlaid, for PKS 1046-409, a CDQ. \Radiocontours{1, 2, 4, 8, 100, 200}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.12}
\figsetgrptitle{3C 275.1}
\figsetplot{3C275.1_lira_paper_count.eps}
\figsetplot{3C275.1_lira_paper_add.eps}
\figsetplot{3C275.1_A_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 275.1, an LDQ. \Radiocontours{0.5, 1, 2, 5, 70}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.13}
\figsetgrptitle{3C 280.1}
\figsetplot{3C280.1_lira_paper_count.eps}
\figsetplot{3C280.1_lira_paper_add.eps}
\figsetplot{3C280.1_D_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 280.1, an LDQ. \Radiocontours{1, 4, 8, 20}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.14}
\figsetgrptitle{PKS 1311-270}
\figsetplot{PKS1311-270_lira_paper_count.eps}
\figsetplot{PKS1311-270_lira_paper_add.eps}
\figsetplot{PKS1311-270_B_lira_post.pdf}
\figsetplot{PKS1311-270_HS_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for PKS 1311-270, a high-redshift quasar.  \Radiocontours{0.5, 4, 10, 20}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.15}
\figsetgrptitle{4C+11.45}
\figsetplot{4C+11.45_lira_paper_count.eps}
\figsetplot{4C+11.45_lira_paper_add.eps}
\figsetplot{4C+11.45_C_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for 4C+11.45, a quasar.\Radiocontours{0.3, 4, 20, 50, 80}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.16}
\figsetgrptitle{Centaurua B}
\figsetplot{CenB_A_lira_paper_count.eps}
\figsetplot{CenB_A_lira_paper_add.eps}
\figsetplot{CenB_A_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the ATCA 8.6 GHz radio contours overlaid, for Centaurus B, an FR-I RG. \Radiocontours{8, 15, 20, 100, 1000}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.17}
\figsetgrptitle{B3 1428+422}
\figsetplot{B3_1428+422_lira_paper_count.eps}
\figsetplot{B3_1428+422_lira_paper_add.eps}
\figsetplot{B3_1428+422_A_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 1.4 GHz radio contours overlaid, for B3 1428+422, a high-redshift quasar. \Radiocontours{ 0.2, 1, 10, 100}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.18}
\figsetgrptitle{3C 334}
\figsetplot{3C334_lira_paper_count.eps}
\figsetplot{3C334_lira_paper_add.eps}
\figsetplot{3C334_B_lira_post.pdf}
\figsetplot{3C334_H_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 334, a quasar. \Radiocontours{0.15, 0.4, 0.7, 5, 10, 40}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.19}
\figsetgrptitle{PKS 2123-463}
\figsetplot{PKS2123-463_count_lira.eps}
\figsetplot{PKS2123-463_add_lira.eps}
\figsetplot{PKS2123-463_A_lira_post.pdf}
\figsetplot{PKS2123-463_jet_lira_post.pdf}
\figsetplot{PKS2123-463_SHS_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for PKS 2123-463, with the ATCA 18 GHz radio contours overlaid, a high redshift quasar. \Radiocontours{1.3, 2, 4}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.20}
\figsetgrptitle{PKS 1402+044}
\figsetplot{PKS1402+044_lira_paper_count.eps}
\figsetplot{PKS1402+044_lira_paper_add.eps}
\figsetplot{PKS1402+044_jet_post.pdf}
\figsetplot{PKS1402+044_hs_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for PKS 1402+044, a high-redshift quasar. \Radiocontours{0.8, 1.5, 8, 40}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.21}
\figsetgrptitle{3C 327.1}
\figsetplot{3C327.1_lira_paper_count.eps}
\figsetplot{3C327.1_lira_paper_add.eps}
\figsetplot{3C327.1_A_lira_post.pdf}
\figsetplot{3C327.1_B_lira_post.pdf}
\figsetgrpnote{Same as in Fig. \ref{fig:results_3C418}, for 3C 327.1, a HERG. We did not measure the offset as there was no statistically significant emission from the chosen ROIs. \Radiocontours{0.5, 2, 10, 25, 40}}
\figsetgrpend

\figsetend

==> fig6set.tex <==
\figsetstart
\figsetnum{6}
\figsettitle{Optical images and SEDs}

\figsetgrpstart
\figsetgrpnum{6.1}
\figsetgrptitle{3C 6.1}
\figsetplot{3C6.1_WFPC2_PC1_F555W_lira_paper.eps}
\figsetplot{3C6.1_NHS+SHS_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 3C 6.1. (a)The HST Wide Field Planeraty Camera 2 (WFCP2) visible image at 5.5 $\times10^{14}$ GHz (5439 \AA) with the VLA 8.6 GHz radio contours overlaid. The left and right panes show NHS and SHS, respectively. Both the hotspots are not detected at this wavelength. (b) The broadband SEDs of NHS and SHS which indicate that X-rays require a second spectral component.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.2}
\figsetgrptitle{3C 17}
\figsetplot{3C17_STIS_F28X50LP_MIRVIS_7219.eps}
\figsetgrpnote{The HST Space Telescope Imaging Spectrograph (STIS) visible image at 4.16 $\times$ 10$^14$ Hz (7216 \AA) of 3C17 overlaid with the VLA 4.86 GHz radio contours. Knots S3.7 and S11.3 are detected in the optical and coincide with the radio.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.3}
\figsetgrptitle{3C 133}
\figsetplot{3C133_NIC2_F160W_lira_paper.eps}
\figsetplot{3C133_knotB_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 3C 133. (a) The HST Near Infrared Camera and Multi-Object Spectrometer-2 (NICMOS-2) infrared image (IR) at 1.87 $\times10^{14}$ GHz (16030 \AA) with the VLA 4.86 GHz radio contours overlaid. (b) The broadband SED of knot B which indicates that the X-ray emission requires a separate spectral component.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.4}
\figsetgrptitle{3C 213.1}
\figsetplot{3C213.1_hst_nic2_f1602w_lira_paper.eps}
\figsetplot{3C213.1_NHS_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 3C 213.1. (a)The HST NICMOS-2 infrared image at 1.87 $\times10^{14}$ GHz (16030 \AA) with the VLA 8.6 GHz radio contours overlaid. The IR emission coincides with the radio peak in NHS. (b) The broadband SED of NHS which indicates that X-rays require a second spectral component.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.5}
\figsetgrptitle{3C 220.2}
\figsetplot{3C220.2_WFC3_IR_F140W_lira_paper.eps}
\figsetplot{3C220.2_SHS_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 3C 220.2. (a) The HST Wide Field Camera-3 (WFC3) IR image at 2.15 $\times10^{14}$ GHz (13922 \AA) with the VLA 8.4 GHz radio contours overlaid. The IR emission coincides with the radio peak in SHS. (b) The broadband SED of SHS which indicates that the X-rays require a separate spectral component.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.6}
\figsetgrptitle{3C 275.1}
\figsetplot{3C275.1_WFPC2_PC1_F675W_lira_paper.eps}
\figsetplot{3C275.1_knotA_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 3C 275.1. (a) The HST WFPC2 visible image at 4.46 $\times10^{14}$ GHz (6717 \AA) with the 8.4 GHz radio contours overlaid. Knot A is not detected at the optical wavelength. (b) The broadband SED of knot A which indicates that X-rays requires a second sepctral component.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.7}
\figsetgrptitle{3C 280.1}
\figsetplot{3C280.1_WFC3_F140W_lira_paper.eps}
\figsetplot{3C280.1_D_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 3C 280.1. (a) The HST WFPC3 IR at 2.15 $\times10^{14}$ GHz (13922 \AA) with the 4.8 GHz radio contours overlaid. Knot D is not detected at the IR wavelength. However, a faint emission is detected further downstream to the edge of the jet where  the jet makes a sharp turn to the south. It is presumably an obstacle (e.g,. a dense gas cloud) which deflects the jet but deeper observations are necessary to confirm this scenario. (b) The broadband SED of knot D where the assumed two-component phenomenological fit was not possible. However, a single component is fit to the radio data which clearly cannot explain the observed X-ray emission.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.8}
\figsetgrptitle{PKS 1311-270}
\figsetplot{PKS1311-270_WFPC2_PC1_F675_lira_paper.eps}
\figsetplot{PKS1311_270_B+HS_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of PKS 1311-270. (a) The HST WFPC2 visible image at 4.46 $\times10^{14}$ GHz (6717 \AA) with the 8.4 GHz radio contours overlaid. Knot B and HS are not detected at this wavelength. (b) The broadband SEDs of B and HS which indicate that the X-ray emission from both the components requires a second spectral component.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.9}
\figsetgrptitle{4C+11.45}
\figsetplot{4C+11.45_WFPC2_PC1_F555W_lira_paper.eps}
\figsetplot{4C+11.45_knotC_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 4C+11.45. (a) The HST WFPC2 visible image at 5.5 $\times10^{14}$ GHz (5439 \AA) with the VLA 8.4 GHz radio contours overlaid. Knot C is not detected at this wavelength. (b) The broadband SED of knot C which indicates that X-rays requires a second spectral component.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.10}
\figsetgrptitle{3C 334}
\figsetplot{3C334_WFPC2_F555W_lira_paper.eps}
\figsetplot{3C334_270_B+H_SED_lira_paper.pdf}
\figsetgrpnote{Results for the optical and spectral analysis of 3C 334. (a) The HST WFPC2 visible image at 5.5 $\times10^{14}$ GHz (5439 \AA) with the VLA 8.4 GHz radio contours overlaid. Knots B and H are not detected at this wavelength. (b) The broadband SEDs of knots B and H which indicates that X-rays from both the components requires a second spectral component.}
\figsetgrpend

\figsetend


==> figset_offset_desc.tex <==
\textbf{3C 6.1} (Fig. \ref{fig:results_3C6.1}) -- This is an FR-II NLRG source with two X-ray hotspots. We find offsets of 0.19\as~(1.46 kpc) in the northern hotspot (NHS) and 0.25\as~(1.66 kpc) in the southern hotspot (SHS) with X-rays lying upstream of the radio.

\textbf{3C 17} (Fig. \ref{fig:results_3C17}): This is an FR-II BLRG source. We adopt the knot names from \citet{Massaro_2009}. The X-ray centroid and radio peak lie within 0.15\as~of each other in knot S3.7. Knots S11.3 and S10.8 show Xf-type projected offsets of 0.15\as~(0.55 kpc) and 0.18\as~(0.6 kpc) respectively. The jet bending at S11.3 presumably produces a internal shock where a strong shock at the bend produces X-rays while a weaker shock downstream produces radio \citep[e.g.,][]{2005MNRAS.360..926W}. \citet{2018ApJS..238...31M} suggest that a dense intracluster medium might be responsible for bending the jet.

\textbf{3C 133} (Fig. \ref{ref:results_3C133}): This is an FR-II HERG source. The X-ray centroid in Knot A, which lies at a 90\degree~projected apparent bend, lies within in 0.15\as~of its radio peak. Despite the X-ray emission from the knots in the inner-jet, we excluded them from the offset analysis as their separation was less than two ASCI-S pixels.

\textbf{0529+075} (Fig. \ref{fig:results_0529+075}): This is a core-dominated quasar. The inner jet makes a sharp apparent bend to the south and later turns to the southeast at knot B where it shows an Xf-offset of 0.56\as~(4.7 kpc).

\textbf{3C 179} (Fig. \ref{fig:results_3C179}): This is a lobe-dominated quasar. The jet branches out into two directions--northwest and southwest--at knot D, where the X-ray centroid lies upstream of the radio peak by 0.16\as~(1.23 kpc). The northwestern branch terminates in a hotspot (HS) while the southwestern one diffuses away. \citet{1992A&A...259L..61A} suggest that a dense inter-galactic medium at D may be responsible for this splashing. The hotspot also shows an Xf-offset of 0.3\as~(2.31 kpc). 

\textbf{4C+25.21} (Fig. \ref{fig:results_4C+25.21}): This is a high-redshift quasar (z=2.68). The X-ray centroid lies within 0.15\as~ of the radio peak in the hotspot. We also detect significant X-ray emission along a putative direction of the jet between the inner jet and the hotspot. This morphology suggests that IC/CMB presumably produces these X-rays (see section \ref{subsec:flux_ratio} for details).

\textbf{TXS 0833+585} (Fig. \ref{fig:results_TXS0833+575}): This is a hight redshift quasar (z=2.1). The X-ray centroid and the radio peak approximately coincide in knot A. In contrast, it lies upstream of the radio in knot B where the jet makes a 90\degree~projected turn to the south. The flux ratio increases with distance from the core and may indicate that IC/CMB dominates the X-ray emission mechanism (see section \ref{subsec:flux_ratio} for details).

\textbf{3C 213.1} (Fig. \ref{fig:results_3C213.1}): This an FR-II source. NHS is detected in radio, optical and X-rays. The X-ray centroid in NHS is within 0.05\as~(0.17 kpc) of the radio peak.

\textbf{3C 220.2} (Fig. \ref{fig:results_3C220.2}): This is a quasar. The X-ray centroid in SHS is within 0.15\as~(1.28 kpc) of its radio peak. However, unlike most of analyzed jet-features, the position angle of the tentative offset lies perpendicular to the putative direction of the jet. This morphology suggests that hot gases on kpc-scales may be emitting the X-rays rather than the hotspot itself.

\textbf{4C+55.17} (Fig. \ref{fig:results_4C+55.17}): The classification for this source is ambiguous. It was initially classified as a quasar while \citet{McConville_2011} suggest that it is a CSO. The X-ray centroid in knot A lies within 0.15\as~(0.14 kpc) of its radio peak. On the other hand, the hotspot (HS) shows an Xf-offset of 0.23\as~(1.84 kpc).

\textbf{PKS 1046-409} (Fig. \ref{fig:results_PKS1046-409}): This is a core-dominated quasar. The jet makes a projected 20\degree~bend to the south at knot C, where the X-ray centroid lies upstream of the radio peak by 0.54\as~(4.65 kpc).

\textbf{3C 275.1} (Fig. \ref{fig:results_3C275.1}): This is a lobe-dominated quasar. We find that knot A shows an Xf-offset offset of 0.65\as~(4.16 kpc).

\textbf{3C 280.1} (Fig. \ref{fig:results_3C280.1}): This is a lobe-dominated quasar. The jet makes a 30\degree~bend to the south at knot D. This knot shows an Xf-offset of 0.54\as~(4.65 kpc).  A bend in the jet at knot D may produce an internal shock and the onset of the bend could create a strong-shock which can produce X-rays while a weaker shock downstream can produce radio \citep[e.g.,][]{2005MNRAS.360..926W}.

\textbf{PKS 1311-270} (Fig. \ref{fig:results_PKS1311-270}): This is a high-redshift quasar (z=2.19). Knot B shows an Xf-offset of 0.25\as~(2.11 kpc). The scenario is slightly complicated in the case of HS. The radio jet makes a 35\degree~projected turn to the northeast before reaching HS.  Although the X-ray centroid lies closer to the core than its radio peak [by 0.24\as~(2.02 kpc)], the offset is inconsistent with the direction of the jet. It is possible that the jet first turns towards the X-ray centroid before reaching the radio hotspot and projection effects create such an appearance. Alternatively, a large-scale hot and diffuse gas may be emitting the X-rays near HS. 

\textbf{4C+11.45} (Fig. \ref{fig:results_4C+11.45}): This is a quasar. The jet makes a 50\degree~projected bend to the southeast at knot C, where the the X-ray centroid lies downstream of the radio peak by 0.19\as~(1.61 kpc).

\textbf{Centaurus B} (Fig. \ref{fig:results_CenB}): This is an FR-I source. Knot A shows an Rf-type offset of 0.57\as~(0.15 kpc). Such an offset is rarely observed in jets with an FR-I type morphology.

\textbf{B3 1428+422} (Fig. \ref{fig:results_B3_1428+422}): This is one of the highest redshift (z=4.7) X-ray jet known to date. We find that the X-ray centroid in its jet-related feature, A, lies within 0.15\as~(1 kpc) of its radio peak.

\textbf{3C 334} (Fig. \ref{fig:results_3C334}): This is a quasar. Knot B shows an Xf-offset of 0.22\as~(1.46 kpc). In contrast, the X-ray centroid in H, where the jet makes a 90\degree~apparent bend to the northeast, lies within 0.15\as~(1 kpc) of its radio peak.

\textbf{3C 418} (Fig. \ref{fig:results_3C418}): This is a quasar. We newly detect jet-linked X-ray emission from knot B using LIRA. See section \ref{subsec:new_detections} for details.

\textbf{PKS 2123-463} (Fig. \ref{fig:results_pks2123-463}): This is a core-dominated quasar. Knot A shows an Rf-type offset of 0.35\as~(3 kpc) while the hotspot shows an Xf-offset of 0.89\as~(7.62 kpc). We also detect significant X-ray emission along the putative direction of the jet between knot A and the hotspot, which, similar to 4C+25.21, suggests that IC/CMB presumably produces these X-rays (see section \ref{subsec:flux_ratio} for details).

\textbf{PKS 1402+044} (Fig. \ref{fig:results_PKS1402+044}): This is a high-redshift quasar (z=3.2). We could not confirm (\textit{p}-value$\leq$0.04) any significant X-ray emission from the jet of this source, unlike the previous authors in \citet{schwartz2019relativistic}.

\textbf{3C 327.1} (Fig. \ref{fig:results_3C327.1}): This is an FR-II source. Similar to PKS 1402+044, contrary to the previous claim in \citet{massaro2013chandra}, we could not confirm (\textit{p}-value$\leq$0.15)  the presence of any significant X-ray emission from its jet.

==> figset_offset_images.tex <==
\begin{figure*}[h]
    \gridline{
        \fig{{3C6.1_lira_paper_count}.eps}{0.25\textwidth}{(a)}
        \fig{{3C6.1_lira_paper_add}.eps}{0.25\textwidth}{(b)}
        \fig{{3C6.1_lira_paper_offset}.eps}{0.5\textwidth}{(c)}
    }
    \gridline{
    \fig{{3C6.1_NHS_lira_post}.pdf}{0.33\textwidth}{(d)}
     \fig{{3C6.1_SHS_lira_post}.pdf}{0.33\textwidth}{(e)}
    }
\caption{Results for the analysis of 3C 6.1, an FR-II NLRG--with the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component. (c) Same as (a) and (b) but zoomed in to NHS (top) and SHS (bottom) respectively. The Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-rays peak closer to the core than the radio in NHS. The jet appears to make a 90 deg turn to the west before reaching SHS where the X-rays peak upstream of the radio. (d)-(e) The distributions of $\xi$ in each ROI  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{1.5, 8, 15, 40} 
\label{fig:results_3C6.1}}
\end{figure*} 

\begin{figure*}[h]
    \gridline{
        \fig{3C17_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{3C17_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{3C17_S3.7_lira_post}.pdf}{0.33\textwidth}{(c)}
     \fig{{3C17_S11.3_lira_post}.pdf}{0.33\textwidth}{(d)}
     \fig{{3C17_S10.8_lira_post}.pdf}{0.33\textwidth}{(e)}
    }
\caption{Same as in Fig. \ref{fig:results_3C418}, for 3C 17, an FR-II BLRG. \Radiocontours{5, 10, 20, 40, 80} \label{fig:results_3C17}}
\end{figure*} 

\begin{figure*}[h]
    \gridline{
        \fig{3C133_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{3C133_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{3C133_B_lira_post.pdf}{0.33\textwidth}{(c)}
    }
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 133, a HERG. \Radiocontours{ 2, 4, 8, 10, 20, 40, 80}\label{ref:results_3C133}}
\end{figure*} 

\begin{figure*}[h]
    \gridline{
        \fig{0529+075_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{0529+075_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{0529+075_B_lira_post.pdf}{0.33\textwidth}{(c)}
    }
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid,, for 0529+075, a highly-superluminal CDQ.  \Radiocontours{1, 2, 3, 4, 8, 20, 100, 1000} \label{fig:results_0529+075}}
\end{figure*} 

\begin{figure*}[h]
    \gridline{
        \fig{3C179_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{3C179_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{3C179_knot_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{3C179_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid,, for 3C 179, an LDQ. \Radiocontours{ 0.3, 2, 4, 8}
\label{fig:results_3C179}}
\end{figure*} 

\begin{figure*}[h]
    \gridline{
        \fig{{4C+25.21_lira_count}.eps}{0.5\textwidth}{(a)}
        \fig{{4C+25.21_lira_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{4C+25.21_B_post}.pdf}{0.33\textwidth}{(c)}
     \fig{{4C+25.21_C_post}.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for 4C+25.21, a high redshift quasar. \Radiocontours{0.5, 2, 4, 8, 20}\label{fig:results_4C+25.21}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{TXS0833+585_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{TXS0833+585_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{TXS0833+585_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{TXS0833+585_B_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for TXS 0833+585, a high-redshift quasar. \Radiocontours{0.34, 0.5, 2, 20, 200}\label{fig:results_TXS0833+575}}
\end{figure*}


\begin{figure*}[!]
    \gridline{
        \fig{{3C213.1_lira_paper_count}.eps}{0.5\textwidth}{(a)}
        \fig{{3C213.1_lira_paper_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{3C213.1_NHS_lira_post}.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for 3C 213.1, an LERG. \Radiocontours{ 0.5, 2, 8, 40}\label{fig:results_3C213.1}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{{3C220.2_lira_paper_count}.eps}{0.5\textwidth}{(a)}
        \fig{{3C220.2_lira_paper_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{3220.2_shs_lira_post}.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for 3C 220.2, a quasar. \Radiocontours{0.5, 2, 5, 20, 80} \label{fig:results_3C220.2}}
\end{figure*} 

\begin{figure*}[h]
    \gridline{
        \fig{{4C+55.17_lira_paper_count}.eps}{0.5\textwidth}{(a)}
        \fig{{4C+55.17_lira_paper_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{4C+55.17_A_lira_post}.pdf}{0.33\textwidth}{(c)}
     \fig{{4C+55.17_HS_lira_post}.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for 4C+55.17, a quasar/FSRQ. \Radiocontours{ 2, 4, 8, 40, 100, 1000} \label{fig:results_4C+55.17}
}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{PKS1046-409_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{PKS1046-409_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{PKS1046-409_C_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the ATCA 19 GHz radio contours overlaid, for PKS 1046-409, a CDQ. \Radiocontours{ 1, 2, 4, 8, 100, 200}\label{fig:results_PKS1046-409}} 
\end{figure*} 

\begin{figure*}[h]
    \gridline{
        \fig{{3C275.1_lira_paper_count}.eps}{0.5\textwidth}{(a)}
        \fig{{3C275.1_lira_paper_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{3C275.1_A_lira_post}.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 275.1, an LDQ. \Radiocontours{ 0.5, 1, 2, 5, 70} 
\label{fig:results_3C275.1}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{{3C280.1_lira_paper_count}.eps}{0.5\textwidth}{(a)}
        \fig{{3C280.1_lira_paper_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{3C280.1_D_lira_post}.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 280.1, an LDQ. \Radiocontours{ 1, 4, 8, 20}\label{fig:results_3C280.1} 
}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{PKS1311-270_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{PKS1311-270_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{PKS1311-270_B_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{PKS1311-270_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for PKS 1311-270, a high-redshift quasar.  \Radiocontours{ 0.5, 4, 10, 20} \label{fig:results_PKS1311-270}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{{4C+11.45_lira_paper_count}.eps}{0.5\textwidth}{(a)}
        \fig{{4C+11.45_lira_paper_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{4C+11.45_C_lira_post}.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for 4C+11.45, a quasar.\Radiocontours{0.3, 4, 20, 50, 80} \label{fig:results_4C+11.45}}
\end{figure*}



\begin{figure*}[h]
    \gridline{
        \fig{CenB_A_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{CenB_A_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{CenB_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the ATCA 8.6 GHz radio contours overlaid, for Centaurus B, an FR-I RG. \Radiocontours{ 8, 15, 20, 100, 1000}\label{fig:results_CenB}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{B3_1428+422_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{B3_1428+422_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{B3_1428+422_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 1.4 GHz radio contours overlaid, for B3 1428+422, a high-redshift quasar. \Radiocontours{ 0.2, 1, 10, 100}\label{fig:results_B3_1428+422}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{3C334_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{3C334_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{3C334_B_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{3C334_H_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for 3C 334, a quasar. \Radiocontours{0.15, 0.4, 0.7, 5, 10, 40}\label{fig:results_3C334}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{PKS2123-463_count_lira.eps}{0.5\textwidth}{(a)}
        \fig{PKS2123-463_add_lira.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{PKS2123-463_A_lira_post.pdf}{0.33\textwidth}{(c)}
    \fig{PKS2123-463_jet_lira_post.pdf}{0.33\textwidth}{(d)}
     \fig{PKS2123-463_SHS_lira_post.pdf}{0.33\textwidth}{(e)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for PKS 2123-463, with the ATCA 18 GHz radio contours overlaid, a high redshift quasar. \Radiocontours{1.3, 2, 4}\label{fig:results_pks2123-463}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{PKS1402+044_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{PKS1402+044_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{PKS1402+044_jet_post.pdf}{0.33\textwidth}{(c)}
     \fig{PKS1402+044_hs_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, with the VLA 4.8 GHz radio contours overlaid, for PKS 1402+044, a high-redshift quasar. \Radiocontours{0.8, 1.5, 8, 40}\label{fig:results_PKS1402+044}}
\end{figure*}

\begin{figure*}[h]
    \gridline{
        \fig{{3C327.1_lira_paper_count}.eps}{0.5\textwidth}{(a)}
        \fig{{3C327.1_lira_paper_add}.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{{3C327.1_A_lira_post}.pdf}{0.33\textwidth}{(c)}
     \fig{{3C327.1_B_lira_post}.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C418}, for 3C 327.1, a HERG. We did not measure the offset as there was no statistically significant emission from the chosen ROIs. \Radiocontours{0.5, 2, 10, 25, 40}\label{fig:results_3C327.1}}
\end{figure*}

==> individua_src_desc.tex <==
\textbf{3C 6.1} (Fig. \ref{fig:results_3C6.1}) -- This is an FR-II NLRG source with two X-ray hotspots. We find projected offsets of 0.19\as~(1.46 kpc) in the northern hotspot (NHS) and 0.25\as~ (1.66 kpc) in the southern hotspot (SHS) with X-rays lying upstream of the radio.

\textbf{3C 17} (Fig. \ref{fig:results_3C17}): This is an FR-II BLRG source. We adopt the knot names from \citet{Massaro_2009}. The X-ray centroid and radio peak lie within 0.15\as~of each other in knot S3.7. Knots S11.3 and S10.8 show Xf-type projected offsets of 0.15\as~(0.55 kpc) and 0.18\as~(0.6 kpc) respectively. The jet bending at S11.3 produces a presmued internal shock where a strong shock at the bend produces X-rays while a weaker shock downstream produces radio \citep[e.g.,][]{2005MNRAS.360..926W}. \citet{2018ApJS..238...31M} suggest that a dense intracluster medium might be responsible for bending the jet. Moreover, the flux ratio decreases along the jet.


\textbf{3C 133}(Fig. \ref{ref:results_3C133}): This is an FR-II HERG source. The X-ray centroid in Knot A, which lies at a 90 deg projected apparent bend, lies within in 0.15\as~of its radio peak. Despite the X-ray emission from the knots in the inner-jet, we excluded them from the offset analysis as their separation was less than two ASCI-S pixels.

\textbf{0529+075}(Fig. \ref{fig:results_0529+075}): This is a core-dominated Quasar. The inner jet makes a sharp apparent bend to the south and later turns to the southeast at knot B where it shows an Xf-type offset of 0.56\as~(4.7 kpc).

\textbf{3C 179}(Fig. \ref{fig:results_3C179}): This is a lobe-dominated Quasar. The jet branches out into two directions--northwest and southwest--at knot D, where the X-ray centroid lies upstream of the radio peak by 0.16\as~(1.23 kpc). The northwestern branch terminates in a hotspot (HS) while the southwestern one diffuses away. \citet{1992A&A...259L..61A} suggest that a dense inter-galactic medium at D may be responsible for this splashing. The hotspot also shows an Xf-offset of 0.3\as~(2.31 kpc). 

\textbf{4C+25.21} (Fig. \ref{fig:results_4C+25.21}): This is a high-redshift quasar (z=2.68). The X-ray centroid lies within 0.15\as~ of the radio peak in the hotspot. We also detect significant X-ray emission along a putative direction of the jet between the inner jet and the hotspot. It suggests that IC/CMB presumably produces these X-rays (see section \ref{subsec:flux_ratio} for details).

\textbf{TXS 0833+585} (Fig. \ref{fig:results_TXS0833+575}): This is a hight redshift Quasar (z=2.1). The X-ray centroid and the radio peak approximately coincide in knot A. In contrast, it lies upstream of the radio in knot B where the jet makes a 90 deg projected turn to the south. The flux ratio increases with distance from the core and may indicate that IC/CMB dominates the X-ray emission mechanism (see section \ref{subsec:flux_ratio} for details).

\textbf{3C 213.1} (Fig. \ref{fig:results_3C213.1}): This an FR-II source. NHS is detected in radio, optical and X-rays. The X-ray centroid in NHS is within 0.05\as~(0.17 kpc) of the radio peak.

\textbf{3C 220.2} (Fig. \ref{fig:results_3C220.2}): This is a Quasar. The X-ray centroid in SHS is within 0.15\as~(1.28 kpc) of its radio peak. 

\textbf{4C+55.17} (Fig. \ref{fig:results_4C+55.17}): This classification of this source is ambiguous. It was initially classified as a Quasar while \citet{McConville_2011} suggest that it is a CSO. The X-ray centroid in knot A lies within 0.15\as~(0.14 kpc) of its radio peak. On the other hand, the hotspot (HS) show an Xf-type projected offset of 0.23\as~(1.84 kpc).

\textbf{PKS 1046-409} (Fig. \ref{ref:results_PKS1046-409}): This is a core-dominated Quasar. The jet makes a projected 20 deg bend to the south at knot C, where the X-ray centroid lies upstream of the radio peak by 0.54\as~(4.65 kpc).

\textbf{3C 275.1} (Fig. \ref{fig:results_3C275.1}): This is a lobe-dominated Quasar. We find that knot A shows an Xf-type offset of 0.65\as~(4.16 kpc).

\textbf{3C 280.1} (Fig. \ref{fig:results_3C280.1}): This is a lobe-dominated quasar. The jet makes a 30 deg bend to the south at knot D. This knot shows an Xf-type offset of 0.54\as~(4.65 kpc).  A bend in the jet at knot D may produce an internal shock and the onset of the bend could create a strong-shock which can produce X-rays while a weaker shock downstream can produce radio \citep[e.g.,][]{2005MNRAS.360..926W}.

\textbf{PKS 1311-270} (Fig. \ref{fig:results_PKS1311-270}): This is a high-redshift Quasar (z=2.19). Knot B shows an Xf-type offset of 0.25\as~(2.11 kpc). The scenario is slightly complicated in the case of HS. The radio jet makes a 35 deg projected turn to the northeast before reaching HS.  Although the X-ray centroid lies closer to the core than its radio peak [by 0.24\as~(2.02 kpc)], the offset is inconsistent the direction of the jet. It is possible that the jet first turns towards the X-ray centroid before reaching the radio hotspot and projection effects create such an appearance. Alternatively, a large-scale hot and diffuse gas may be emitting the X-rays near HS. 

\textbf{4C+11.45} (Fig. \ref{fig:results_4C+11.45}): This is a Quasar. The jet makes a 50 deg projected bend to the southeast at knot C, where the the X-ray centroid lies downstream of the radio peak by 0.19\as~(1.61 kpc).

\textbf{Centaurus B} (Fig. \ref{fig:results_CenB}): This is an FR-I source. Knot A shows an Rf-type offset of 0.57\as~(0.15 kpc). Such an offset is rarely observed in jets with FR-I type morphologies.

\textbf{PKS 1402+044} (Fig. \ref{fig:results_PKS1402+044}): This is a high-redshift Quasar (z=3.2). We could not confirm (\textit{p}-value=0.04) any significant X-ray emission from the jet of this source, unlike the previous authors in \citet{schwartz2019relativistic}.

\textbf{B3 1428+422} (Fig. \ref{fig:results_B3_1428+422}): This is one of the highest redshift (z=4.7) X-ray jet known to date. We find that the X-ray centroid in its jet-related feature, A, lies within 0.15\as~(1 kpc) of its radio peak.

\textbf{3C 327.1} (Fig. \ref{fig:results_3C327.1}): This is an FR-II source. Similar to PKS 1402+044, contrary to the previous claim in \citet{massaro2013chandra}, we could not confirm the presence of any significant X-ray emission from its jet.

\textbf{3C 334} (Fig. \ref{fig:results_3C334}): This is a Quasar. Knot B shows an Xf-type offset of 0.22\as~(1.46 kpc). In contrast, the X-ray centroid in H, where the jet makes a 90 deg apparent bend to the northeast, lies within 0.15\as~(1 kpc) of its radio peak.

\textbf{3C 418} (Fig. \ref{fig:results_3C418}): This is a Quasar. We newly detect jet-linked X-ray emission from knot B using LIRA. Unlike other offsets, the X-ray peaks to the edge of the jet near knot B. The jet also makes a 60 deg projected bend to the north at this knot. This morphology suggests the jet itself may not be producing the observed X-ray emission. It may instead be originating from a jet-deflecting stationary obstacle (e.g., a dense gas cloud), which gets shock-heated by the jet (e.g., via entrainment). Hence, deeper multi-wavelength observations are necessary to establish the true nature of this X-ray emission.

\textbf{PKS 2123-463} (Fig. \ref{fig:results_pks2123-463}): This is a core-dominated Quasar. Knot A shows an Rf-type offset of 0.35\as~(3 kpc) while the hotspot shows an Xf-type offset of 0.89\as~(7.62 kpc). We also detect significant X-ray emission along the putative direction of the jet between knot A and the hotspot, which, similar to 4C+25.21, suggests that IC/CMB presumably produces these X-rays (see section \ref{subsec:flux_ratio} for details).

==> obs_data.tex <==
\startlongtable
\begin{deluxetable*}{ccccCccc}
  \tablecaption{Observations and Imaging data\label{table:radio_xray_obs}}
  \tabletypesize{\scriptsize}
  \tablehead{
    \colhead{IAU Name} &
    \multicolumn{1}{p{2cm}}{\centering Radio\\project code} &
    \colhead{Date}&
    \multicolumn{1}{p{1.5cm}}{\centering Frequency\\GHz} &
    \multicolumn{1}{p{2cm}}{\centering Beam size\\\arcsec$\times$\arcsec} &
    \multicolumn{1}{p{1cm}}{\centering Chandra\\ObsID} &
    \multicolumn{1}{p{2cm}}{\centering Effective\\exposure (ks)} &
    \colhead{\texttt{blur}}
  }
  \startdata
       3C 6.1    &    AP0380    &    1999 Aug 02    &    8.4    &    0.25\times0.24    &    3009    &    33.7    &    0.3\\
3C 17    &    AS0179    &    1985 Mar 08    &    4.8    &    0.48\times0.39    &    9292    &    7.9    &    0.3\\
3C 133    &    AL0164    &    1987 Oct 09    &    4.8    &    0.39\times0.36    &    9300    &    7    &    0.25\\
0529+075    &    AH0824    &    2003 Aug 12    &    4.8    &    0.42\times0.35    &    9289    &    8.7    &    0.3\\
3C 179    &    AA0149    &    1992 Nov 10    &    8.4    &    0.29\times0.19    &    2123    &    8.6    &    0.3\\
4C+25.21 & AK0353 & 1994 Mar 21 & 8.4 & 0.30\times0.21 & 10307 & 19.8 & 0.25\\
TXS 0833+585    &    AL0164    &    1987 Oct 09    &    4.8    &    0.43\times0.38    &    7870    &    3.8    &    0.28\\
3C 213.1 & AS0179 & 1985 Mar 03 & 4.8 & 1.12\times0.46&9307 & 7.6 & 0.28\\
3C 220.2    &    AK0403    &    1995 Jul 27    &    8.4    &    0.33\times0.23    &    18098    &    11.4    &    0.3\\
4C+55.17    &    AM0672    &    2000 Nov 05    &    8.4    &    0.40\times0.21    &    4842    &    28    &    0.25\\
PKS 1046-409    &    C890 (ATCA)    &    2004 May 12    &    19    &    0.73\times0.48    &    3116    &    3.8    &    0.25\\
3C 275.1    &    AG0247    &    1987 Sep 14    &    4.8    &    0.42\times0.40    &    2096    &    21    &    0.2\\
3C 280.1 & AK0180 & 1987 Jul 26 & 4.8 & 0.47\times0.41 & 21398 & 15.8 & 0.25\\
PKS 1311-270    &    AK0353    &    1994 Mar 21    &    8.4    &    0.44\times0.23    &    10306    &    17.9    &    0.3\\
4C+11.45    &    AK0353    &    1994 Mar 21    &    8.4    &    0.30\times0.23    &    10310    &    17.8    &    0.27\\
Centaurus B    &    C890 (ATCA)    &    2002 Feb 02    &    8.6    &    1.35\times1.28    &    3120    &    3.7    &    0.25\\
B3 1428+422    &    AC0755    &    2004 Dec 06    &    1.4    &    1.82\times1.39    &    7874    &    7    &    0.25\\
3C 334    &    AB0369    &    1986 May 05    &    4.8    &    0.40\times0.38    &    2097    &    17.6    &    0.25\\
3C 327.1    &    AM0548    &    1996 Oct 26    &    4.8    &    0.41\times0.38    &    13887    &    10.3    &    0.28\\
3C 418 & AF0376 & 2000 Dec 10 & 8.4 & 0.24\times0.23 & 21401 & 17.8 & 0.25\\
2123-463    &    C890 (ATCA)    &   2004 May 10     &   17.7     &     0.5\times0.5   &    4890    &    6.47    &    0.28\\
         \enddata
        \end{deluxetable*}

 

==> offset_images.tex <==
\section{Results for offset analysis}
\FloatBarrier
\begin{figure*}[h]
    \gridline{
        \fig{images/lira_outputs/3C6.1_lira_paper_count.eps}{0.25\textwidth}{(a)}
        \fig{images/lira_outputs/3C6.1_lira_paper_add.eps}{0.25\textwidth}{(b)}
        \fig{images/lira_outputs/3C6.1_lira_paper_offset.eps}{0.5\textwidth}{(c)}
    }
    \gridline{
    \fig{images/lira_outputs/3C6.1_NHS_lira_post.pdf}{0.33\textwidth}{(d)}
     \fig{images/lira_outputs/3C6.1_SHS_lira_post.pdf}{0.33\textwidth}{(e)}
    }
\caption{Results for the analysis of 3C 6.1, an FR-II NLRG--with the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component. (c) Same as (a) and (b) but zoomed in to NHS (top) and SHS (bottom) respectively. The Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-rays peak closer to the core than the radio in NHS. The jet appears to make a 90 deg turn to the west before reaching SHS where the X-rays peak upstream of the radio.

. (d)-(e) The distributions of $\xi$ in each ROI  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{1.5, 8, 15, 40} 
\label{fig:results_3C6.1}}
\end{figure*} 



\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C17_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C17_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C17_S3.7_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C17_S11.3_lira_post.pdf}{0.33\textwidth}{(d)}
     \fig{images/lira_outputs/3C17_S10.8_lira_post.pdf}{0.33\textwidth}{(e)}
    }
\caption{Results for the analysis of 3C 17, am FR-II BLRG. With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green).  (c)-(e) The distributions of $\xi$ in each ROI  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{5, 10, 20, 40, 80} \label{ref:results_3C17}}

\end{figure*} 


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C133_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C133_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C133_B_lira_post.pdf}{0.33\textwidth}{(c)}
    }
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 133, a HERG. \Radiocontours{ 2, 4, 8, 10, 20, 40, 80}\label{ref:results_3C133}}
\end{figure*} 


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/0529+075_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/0529+075_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/0529+075_B_lira_post.pdf}{0.33\textwidth}{(c)}
    }
\caption{Same as in Fig. \ref{fig:results_3C17}, for 0529+075, a highly-superluminal CDQ.  \Radiocontours{1, 2, 3, 4, 8, 20, 100, 1000} \label{ref:results_0529+075}}

\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C179_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C179_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C179_knot_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C179_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 179, an LDQ. \Radiocontours{ 0.3, 2, 4, 8}
\label{fig:results_3C179}}

\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/4C+25.21_lira_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/4C+25.21_lira_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/4C+25.21_B_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/4C+25.21_C_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 4C+25.21, a high redshift Quasar. \Radiocontours{0.5, 2, 4, 8, 20}\label{fig:results_4C+25.21}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/TXS0833+585_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/TXS0833+585_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/TXS0833+585_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/TXS0833+585_B_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for TXS 0833+585, a high-redshift Quasar. \Radiocontours{0.34, 0.5, 2, 20, 200}\label{fig:results_TXS0833+575}}

 
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C213.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C213.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C213.1_NHS_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 213.1, an LERG. \Radiocontours{ 0.5, 2, 8, 40}\label{fig:results_3C213.1}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C220.2_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C220.2_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3220.2_shs_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 220.2, a Quasar. \Radiocontours{0.5, 2, 5, 20, 80} \label{fig:results_3C220.2}}
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/4C+55.17_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/4C+55.17_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/4C+55.17_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/4C+55.17_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 4C+55.17, a Quasar/FSRQ. \Radiocontours{ 2, 4, 8, 40, 100, 1000} \label{fig:results_4C+55.17}
}
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS1046-409_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS1046-409_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS1046-409_C_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for PKS 1046-409, a CDQ. \Radiocontours{ 1, 2, 4, 8, 100, 200}\label{fig:results_PKS1046-409}} 
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C275.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C275.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C275.1_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 275.1, an LDQ. \Radiocontours{ 0.5, 1, 2, 5, 70} 
\label{fig:results_3C275.1}}
\end{figure*}


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C280.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C280.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C280.1_D_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 280.1, an LDQ. \Radiocontours{ 1, 4, 8, 20}\label{fig:results_3C280.1} 
}
\end{figure*}


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS1311-270_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS1311-270_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS1311-270_B_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/PKS1311-270_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for PKS 1311-270, a high-redshift Quasar.  \Radiocontours{ 0.5, 4, 10, 20} \label{fig:results_PKS1311-270}}
\end{figure*}


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/4C+11.45_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/4C+11.45_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/4C+11.45_C_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 4C+11.45, a Quasar.\Radiocontours{0.3, 4, 20, 50, 80} \label{fig:results_4C+11.45}}
 
\end{figure*}



\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/CenB_A_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/CenB_A_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/CenB_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for Centaurus B, an FR-I RG. \Radiocontours{ 8, 15, 20, 100, 1000}\label{fig:results_CenB}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/B3_1428+422_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/B3_1428+422_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/B3_1428+422_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for B3 1428+422, a hight-redshift Quasar. \Radiocontours{ 0.2, 1, 10, 100}\label{fig:results_B3_1428+422}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C334_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C334_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C334_B_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C334_H_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 334, a Quasar. \Radiocontours{0.15, 0.4, 0.7, 5, 10, 40}\label{fig:results_3C334}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C418_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C418_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C418_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C418_B_lira_post.pdf}{0.33\textwidth}{(d)}
      \fig{images/lira_outputs/3C418_C_lira_post.pdf}{0.33\textwidth}{(e)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 418, a Quasar. \Radiocontours{ 2, 4, 8, 15} \label{fig:results_3C418}}
\end{figure*}


    

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS2123-463_count_lira.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS2123-463_add_lira.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS2123-463_A_lira_post.pdf}{0.33\textwidth}{(c)}
    \fig{images/lira_outputs/PKS2123-463_jet_lira_post.pdf}{0.33\textwidth}{(d)}
     \fig{images/lira_outputs/PKS2123-463_SHS_lira_post.pdf}{0.33\textwidth}{(e)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for PKS 2123-463, a high redshift Quasar. \Radiocontours{1.3, 2, 4}\label{fig:results_pks2123-463}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C327.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C327.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C327.1_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C327.1_B_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for 3C 327.1, a HERG. We did not measure the offset as there was no statistically significant emission from the chosen ROIs. \Radiocontours{0.5, 2, 10, 25, 40}\label{fig:results_3C327.1}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS1402+044_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS1402+044_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS1402+044_jet_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/PKS1402+044_hs_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Same as in Fig. \ref{fig:results_3C17}, for PKS 1402+044, a high-redshift Quasar. \Radiocontours{0.8, 1.5, 8, 40}\label{fig:results_PKS1402+044}}
\end{figure*}












==> offset_images_old.tex <==
\restartappendixnumbering
\appendix
\section{Results for offset analysis}
\FloatBarrier
\begin{figure*}[h]
    \gridline{
        \fig{images/lira_outputs/3C6.1_lira_paper_count.eps}{0.25\textwidth}{(a)}
        \fig{images/lira_outputs/3C6.1_lira_paper_add.eps}{0.25\textwidth}{(b)}
        \fig{images/lira_outputs/3C6.1_lira_paper_offset.eps}{0.5\textwidth}{(c)}
    }
    \gridline{
    \fig{images/lira_outputs/3C6.1_NHS_lira_post.pdf}{0.33\textwidth}{(d)}
     \fig{images/lira_outputs/3C6.1_SHS_lira_post.pdf}{0.33\textwidth}{(e)}
    }
\caption{Results for the analysis of 3C 6.1, an FR-II NLRG--with the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component. (c) Same as (a) and (b) but zoomed in to NHS (top) and SHS (bottom) respectively. The Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-rays peak closer to the core than the radio in NHS. The jet appears to make a 90 deg turn to the west before reaching SHS where the X-rays peak upstream of the radio.
. (d)-(e) The distributions of $\xi$ in each ROI  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{1.5, 8, 15, 40} 
\label{fig:results_3C6.1}}
\end{figure*} 


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C17_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C17_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C17_S3.7_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C17_S11.3_lira_post.pdf}{0.33\textwidth}{(d)}
     \fig{images/lira_outputs/3C17_S10.8_lira_post.pdf}{0.33\textwidth}{(e)}
    }
\caption{Results for the analysis of 3C 17, am FR-II BLRG. We adopt the knot names from \citet{Massaro_2009} and with the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). In addition to the reported X-ray knots in \citet{Massaro_2009}, we also find significant evidence for X-ray emission from knot S10.9. The X-ray centroid in S3.7 approximately coincides with its corresponding radio peak. In contrast, it lies upstream in both S11.3 and S10.8. The jet bending at S11.3 presumably produces an internal shock where a strong shock at the bend produces X-rays while a weaker shock downstream produces radio \citep[e.g.,][]{2005MNRAS.360..926W}. \citet{2018ApJS..238...31M} suggest that a dense intra-cluster medium might be responsible for bending the jet. (c)-(e) The distributions of $\xi$ in each ROI  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{5, 10, 20, 40, 80} \label{ref:results_3C17}}
\end{figure*} 


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C133_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C133_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C133_B_lira_post.pdf}{0.33\textwidth}{(c)}
    }
\caption{Results for the analysis of 3C 133, a HERG--With the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within the ROI, B (dashed-green).  The jet makes a projected 90 deg bend to the south at knot B where the X-ray centroid and the radio peak approximately coincide. (c) The distributions of $\xi$ in B  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{ 2, 4, 8, 10, 20, 40, 80}\label{ref:results_3C133}}
\end{figure*} 


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/0529+075_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/0529+075_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/0529+075_B_lira_post.pdf}{0.33\textwidth}{(c)}
    }
\caption{Results for the analysis of 0529+075, a highly-superluminal CDQ--with the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within the ROI, B (dashed-green).  The inner jet makes a sharp apparent bend to the south and later turns to the southeast at knot B. The X-ray centroid at B lies upstream of the radio peak.  (c) The distributions of $\xi$ in B  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve).  \Radiocontours{1, 2, 3, 4, 8, 20, 100, 1000} \label{ref:results_0529+075}}
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C179_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C179_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C179_knot_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C179_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of 3C 179, an LDQ--With the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The jet branches out in to two directions--northwest and southwest--at knot D where the X-ray centroid lies upstream of the radio peak where. The northwestern branch terminates in a hotspot (HS) while the southwestern one diffuses away. \citet{1992A&A...259L..61A} suggest that a dense inter-galactic medium at D may be responsible for this splashing. The X-ray centroid also lies upstream of the radio in HS. (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{ 0.3, 2, 4, 8}
\label{fig:results_3C179}}
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/4C+25.21_lira_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/4C+25.21_lira_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/4C+25.21_B_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/4C+25.21_C_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of 4C+25.21, a high redshift Quasar--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-ray centroid in the hotspot coincides with the radio emission. We also detect significant X-ray emission along the putative direction of the jet between the inner jet and the hotspot, which suggests that IC/CMB presumably produces these X-rays (see section \ref{subsec:flux_ratio} for details). (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{0.5, 2, 4, 8, 20}\label{fig:results_4C+25.21}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/TXS0833+585_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/TXS0833+585_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/TXS0833+585_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/TXS0833+585_B_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of TXS 0833+585, a high-redshift quasar--With the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-ray centroid and the radio peak approximately coincide in knot A. In contrast it lies upstream of the radio in knot B where the jet makes a 90 deg projected turn to the south. (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{0.34, 0.5, 2, 20, 200}\label{fig:results_TXS0833+575}}

 
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C213.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C213.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C213.1_NHS_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of 3C 213.1, an LERG--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within the ROI, NHS (dashed-green). The X-ray centroid in NHS coincides with the radio peak in NHS. (c) The distributions of $\xi$ in NHS  for the observed image (blue-shaded), 50 simulated images of the baseline model (gray) and their average (gray-shaded area with a dashed-black curve). \Radiocontours{ 0.5, 2, 8, 40}\label{fig:results_3C213.1}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C220.2_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C220.2_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3220.2_shs_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of 3C 220.2, a quasar--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within in the ROI, SHS (dashed-green). The X-ray centroid approximately coincides with the radio peak. (c) The distributions of $\xi$ in SHS  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{0.5, 2, 5, 20, 80} \label{fig:results_3C220.2}}
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/4C+55.17_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/4C+55.17_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/4C+55.17_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/4C+55.17_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of 4C+55.17, a quasar/FSRQ--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-ray centroid in knot A approximately coincides with its corresponding radio peak but it lies upstream in HS.  (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{ 2, 4, 8, 40, 100, 1000} \label{fig:results_4C+55.17}
}
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS1046-409_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS1046-409_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS1046-409_C_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of PKS 1046-409, a CDQ--With the ATCA 19 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within the ROI, C (dashed-green). The jet makes a projected 20deg bend to the south at C where the X-ray centroid lies upstream of the radio peak. (c) The distributions of $\xi$ in C  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{ 1, 2, 4, 8, 100, 200}\label{fig:results_PKS1046-409}} 
\end{figure*} 

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C275.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C275.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C275.1_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of 3C 275.1, an LDQ--With the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within in ROI, A (dashed-green). The X-ray centroid in A lies upstream of its radio peak. (c) The distributions of $\xi$ in A  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{ 0.5, 1, 2, 5, 70} 
\label{fig:results_3C275.1}}
\end{figure*}


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C280.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C280.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C280.1_D_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of 3C 280.1, an LDQ--With the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within in the ROI, D (dashed-green). The jet makes a 30 deg bend to the south at knot D. Here the X-rays peak upstream of the radio. It is possible that a bend in the jet at knot D produces an internal shock. The onset of the bend could create a strong-shock which can produce X-rays while a weaker shock downstream can produce radio \citep[e.g.,][]{2005MNRAS.360..926W}. (c) The distributions of $\xi$ in A  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{ 1, 4, 8, 20}\label{fig:results_3C280.1} 
}
\end{figure*}


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS1311-270_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS1311-270_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS1311-270_B_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/PKS1311-270_HS_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of PKS 1311-270, a high-redshift quasar--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-ray centroid in knot B lies upstream of its radio peak. The scenario is slightly complicated in the case of HS. The radio jet which makes a 35 deg projected turn to the northeast before reaching HS. However, the X-ray centroid, although lies closer to the core than its corresponding radio peak, is not consistent with the putative direction of the jet. It is possible that the jet first turns towards the X-ray centroid before reaching the radio hotspot and projection effects create such an appearance. Alternatively, a large-scale hot, diffuse gas may be emitting the X-rays at HS.  (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve).  \Radiocontours{ 0.5, 4, 10, 20} \label{fig:results_PKS1311-270}}
\end{figure*}


\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/4C+11.45_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/4C+11.45_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/4C+11.45_C_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of 4C+11.45, a quasar--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within in ROI, C (dashed-green). The jet makes a 50 deg projected bend to the southeast at knot C where the the X-ray centroid lies downstream of the radio peak. (c) The distributions of $\xi$ in C  for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve)\Radiocontours{0.3, 4, 20, 50, 80} \label{fig:results_4C+11.45}}
 
\end{figure*}



\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/CenB_A_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/CenB_A_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/CenB_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of Centaurus B, an FR-I RG--With the ATCA 8.6 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within in ROI A (dashed-green). The X-ray centroid in A lies downstream of the radio peak. (c) The distributions of $\xi$ in A for the observed image (blue-shaded), 50 simulated images of the baseline model (gray) and their average (gray-shaded area with a dashed-black curve). \Radiocontours{ 8, 15, 20, 100, 1000}\label{fig:results_CenB}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/B3_1428+422_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/B3_1428+422_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/B3_1428+422_A_lira_post.pdf}{0.33\textwidth}{(c)}
    }
    
\caption{Results for the analysis of B3 1428+422, a hight-redshift quasar--With the VLA 1.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within the ROI, A (dashed-green). The X-ray centroid in A approximately coincides with its radio peak. If we adopt the estimated bulk Lorentz factor $\Gamma\approx5-10$ \citep[e.g.,][]{2010A&A...521A...6V} (under the IC/CMB model), any existing offset would be reduced by a factor of at least 3 and combined with a high redshift (z=4.715), it may not be resolvable. (c) The distributions of $\xi$ in A  for the observed image (blue-shaded), 50 simulated images of the baseline model (gray) and their average (gray-shaded area with a dashed-black curve). \Radiocontours{ 0.2, 1, 10, 100}\label{fig:results_B3_1428+422}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C334_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C334_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C334_B_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C334_H_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of 3C 334, a quasar--With the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-ray centroid in B lies upstream of its radio peak. In contrast, the X-ray centroid in H, where the jet makes a 90 deg apparent bend to the northeast, approximately coincides with its radio peak. (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{0.15, 0.4, 0.7, 5, 10, 40}\label{fig:results_3C334}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C418_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C418_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C418_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C418_B_lira_post.pdf}{0.33\textwidth}{(d)}
      \fig{images/lira_outputs/3C418_C_lira_post.pdf}{0.33\textwidth}{(e)}
    }
    
\caption{Results for the analysis of 3C 418, a quasar--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within the ROI, B (dashed-green).  Unlike most of the offsets reported in this work, the X-ray peaks to the edge of the jet, adjacent to the radio peak in knot B. The jet also makes a 60 deg projected bend to the north at this knot. This suggests that the jet itself may not be producing the observed X-ray emission. It may instead be originating from a jet-deflecting stationary obstacle (e.g., a dense gas cloud), which gets shock heated by the jet (e.g., by entrainment). Deeper multi-wavelength observations are necessary to confirm this scenario. (c)-(e) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). We only detect statistically significant emission from ROI, B. \Radiocontours{ 2, 4, 8, 15} \label{fig:results_3C418}}
\end{figure*}


    

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS2123-463_count_lira.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS2123-463_add_lira.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS2123-463_A_lira_post.pdf}{0.33\textwidth}{(c)}
    \fig{images/lira_outputs/PKS2123-463_jet_lira_post.pdf}{0.33\textwidth}{(d)}
     \fig{images/lira_outputs/PKS2123-463_SHS_lira_post.pdf}{0.33\textwidth}{(e)}
    }
    
\caption{Results for the analysis of PKS 2123-463, a high redshift Quasar--With the ATCA 18 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). The X-ray centroid lies downstream of its radio peak in A while it lies upstream in HS. We also detect significant X-ray emission along the putative direction of the jet between knot A and the hotspot, which, similar to 4C+25.21, suggests that IC/CMB presumably produces these X-rays (see section \ref{subsec:flux_ratio} for details). (c)-(e) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). \Radiocontours{1.3, 2, 4}\label{fig:results_pks2123-463}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/3C327.1_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/3C327.1_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/3C327.1_A_lira_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/3C327.1_B_lira_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of 3C 327.1, a HERG--With the VLA 8.4 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). Contrary to what is reported in its detection paper, we did not find significant evidence for X-ray emission from the jet. \Radiocontours{0.5, 2, 10, 25, 40}\label{fig:results_3C327.1}}
\end{figure*}

\begin{figure*}
    \gridline{
        \fig{images/lira_outputs/PKS1402+044_lira_paper_count.eps}{0.5\textwidth}{(a)}
        \fig{images/lira_outputs/PKS1402+044_lira_paper_add.eps}{0.5\textwidth}{(b)}
    }
    \gridline{
    \fig{images/lira_outputs/PKS1402+044_jet_post.pdf}{0.33\textwidth}{(c)}
     \fig{images/lira_outputs/PKS1402+044_hs_post.pdf}{0.33\textwidth}{(d)}
    }
    
\caption{Results for the analysis of PKS 1402+044, a quasar--With the VLA 4.8 GHz radio contours overlaid in the top panel--(a) The \textit{Chandra} observation, binned by a factor of 0.5. (b) The average added component where the Red \texttt{X} marks the centroid of the added component within each ROI (dashed-green). (c)-(d) The distributions of $\xi$ in each ROI for the observed image (shaded blue), 50 simulated images of the baseline model (gray) and their average (gray shaded area with a dashed-black curve). Similar to 3C 327.1, we did not find any significant evidence for X-ray emission from the jet as opposed to what is reported. \Radiocontours{0.8, 1.5, 8, 40}\label{fig:results_PKS1402+044}}
\end{figure*}











